Parallel Programming for FPGAs

This book focuses on the use of algorithmic high-level synthesis (HLS) to build application-specific FPGA systems. Our goal is to give the reader an appreciation of the process of creating an optimized hardware design using HLS. Although the details are, of necessity, different from parallel programming for multicore processors or GPUs, many of the fundamental concepts are similar. For example, designers must understand memory hierarchy and bandwidth, spatial and temporal locality of reference, parallelism, and tradeoffs between computation and storage. This book is a practical guide for anyone interested in building FPGA systems. In a university environment, it is appropriate for advanced undergraduate and graduate courses. At the same time, it is also useful for practicing system designers and embedded programmers. The book assumes the reader has a working knowledge of C/C++ and includes a significant amount of sample code. In addition, we assume familiarity with basic computer architecture concepts (pipelining, speedup, Amdahl's Law, etc.). A knowledge of the RTL-based FPGA design flow is helpful, although not required.

==> cookbook.tex <==





==> dft_project.tex <==
\chapter{Discrete Fourier Transform (DFT) Project}
\glsresetall
\label{chapter:DFT_project}

\section{Introduction}
The goal of this project is design architectures that implement the Discrete Fourier Transform (DFT).  The DFT is a common operation in signal processing which generates a frequency domain representation of the discrete input signal. We start with the direct implementation of the DFT which is a matrix-vector multiplication. The input signal is a vector of samples and the matrix is composed of a set of basis functions corresponding to discrete cosine and sine waveforms of different frequencies. The multiplication of the input signal with these basis functions describes how well the input signal correlates with those waveforms, which is the value of the Fourier series at that frequency.

\section{Materials}
You can find the following files in \texttt{project2-dft.zip}. These are divided into four folders: \texttt{dft\_8\_precomputed}, \texttt{dft\_32\_precomputed}, \texttt{dft\_256\_precomputed}, and \texttt{dft\_1024\_precomputed}. Each of these folders has its own testbench, \texttt{out.gold.dat} file, and \texttt{coefficients.h} file. 

Each folder contains following files:
\begin{itemize}
\item \texttt{dft.cpp}: The baseline implementation for the dft function.
\item \texttt{dft.h}: Header file holding important constants and other variables.
\item \texttt{dft\_test.cpp}: Testbench
\item \texttt{coefficientsX.h}: A file containing the values of corresponding to one sine/cosine period sampled based upon the DFT points. For example, an 8 point DFT has 8 samples across both the sine and cosine function evenly spaced across one period. This is equivalent to dividing one rotation in the complex plane equally by the number of points in the DFT. 
\item \texttt{out.gold.dat}: ``Golden'' output. The testbench (dft\_test.cpp) generates a sample input and calls the function \texttt{dft} in \texttt{dft.cpp} with that sample input. This output of the function is compared to the expected output. This will indicate PASS or FAIL. If it fails, then the code in \texttt{dft} is incorrect. There are four different versions of depending on the DFT size and way in which the DFT coefficients were generated.
\item \texttt{script.tcl} and \texttt{directives.tcl}: Used to create the project. 
\end{itemize}

\section{Project Goal}
You should modify the code to create a number of different architectures that perform tradeoffs between performance and area.  For \texttt{dft\_256\_precomputed} and \texttt{dft\_1024\_precomputed} designs, you need to use precomputed values from \texttt{coefficients256.h} and \texttt{coefficients1024.h}. 

For 256-point and 1024-point DFTs, you will create a report describing how you generated these different architectures (code restructuring, pragmas utilized, etc.). For each architecture you should provide its results including the resource utilization (BRAMs, DSP48, LUT, FF), and performance in terms of throughput (number of FFT operations/second), latency, clock cycles, clock frequency (which is fixed to 10 ns). You can do most of the design space exploration on the 256 point DFT. You should pick your ``best'' 256 architecture and synthesize that as a 1024 DFT.

The 8 and 32 point folders are provided for your convenience. If you would like, you can do some of your initial design space optimization on these smaller architectures. But it is not necessary to use these at all.

The key in this project is to understand the tradeoffs between loop optimizations (unrolling and pipelining) and data partitioning. Therefore you should focus on these optimizations.

\section{Optimization Hints and Guidelines}
\begin{itemize}
\item You should use a clock period of 10 ns.
\item The output of your architecture must closely match the golden output. Be sure to generate a working function before performing any optimizations. If the result does not match exactly, but is close, please explain why in the report.
\item You should use float for all data types. You do not need to perform bitwidth optimization of this project.
\item The current design is set up to do the DFT in-place, i.e., you put the output results back into the same arrays that give you the input results. You can change this if you think it will give you better results.
\item There are many different ways to generate the DFT coefficients. These are constants when the DFT size is fixed. We have given you the coefficients for both 256 (in \texttt{coefficients256.h}) and 1024 (in \texttt{coefficients1024.h}). They each have two constant arrays, \texttt{sin\_table} and \texttt{cos\_table}. You can use these coefficient arrays directly as memories in your architectures. You are also free to create your own arrays using a different structure (e.g., 2D array, reordering of elements in the given 1D arrays, etc.). Or you could dynamically generate the coefficients. 
\item There is significant amount of parallelism that can be exploited by (partially) unrolling the for loops. Pipelining these (partially) unrolled for loops should lead to higher throughputs.
\item There are more efficient methods for performing the DFT that exploit the symmetries of the Fourier constants, e.g., the fast Fourier transform (FFT). Do not use these symmetries. In other words, treat this like a matrix-vector multiply with unknown matrix values. Do not worry, we will implement FFT architectures in a following project that will fully take advantage of these symmetries.
\item You do not need to report your optimizations for your 8 point and 32 point DFT; these folders are provided for your convenience. Since these will very likely synthesize much faster than larger point DFT functions, it may be useful to use these to debug your code or in your initial design space exploration.
\item Your report must explicitly state how you calculated the throughput results. Note that this is often not simply a function of the latency and the clock period, and involves using the initiation interval.
\end{itemize}

==> emulator.tex <==
\chapter{Wireless Channel Emulator}
\glsresetall
\label{chapter:emulator}

\note{Go through the example wireless channel emulator that we developed.}

==> fir_project.tex <==
\chapter{Finite Impulse Response (FIR) Filter Project}
\glsresetall
\label{chapter:FIR_Project}

\section{Introduction}

In this project, you will do three tasks using \VHLS tool and the Zedboard:
\begin{itemize}
\item Design 11 tap FIR filter
\item Demonstrate the 11 tap filter on the Zedboard
\item Design and optimize 128 tap matched filter. 
\end{itemize}

We provide baseline code for the designs and demo. For the 11 tap FIR filter and demo, you must acquire necessary knowledge from the resources provided with this document. For the matched filter, you must perform necessary optimizations to increase the throughput, decrease the latency, and decrease the area. In your report, you must provide the synthesizable code, describe the optimizations and their architectures, and discuss the impact of each optimization on the throughput, latency, and area.

\section{Preparation}
Before you start, we strongly suggest that you go through these high level synthesis tutorials: Lab 1, Lab 2 and Lab 3 in this document: ug871-vivado-high-level-synthesis-tutorial.pdf. You can find this document in the given Tutorial folder. \note{Fix this. Add this document somewhere and point to it.}

\section{Materials}

\note{Need to add a location for this.}
You can find the following files in project1-fir.zip:
\begin{itemize}
\item \texttt{fir11} folder: 11 tap fir filter
\begin{itemize}
\item \texttt{fir.cpp}: Implements top level function
\item \texttt{fir.h}: Header file
\item \texttt{fir\_test.cpp}: Test bench
\item \texttt{input.dat}: Input chirp signal
\item \texttt{out.gold.dat}: ``Golden'' output. When the testbench (from fir\_test.cpp) is run through the file fir.cpp it should generate this result. If it does not, you did something wrong.
\end{itemize}
\item \texttt{fir128} folder: 128 tap matched filter
\begin{itemize}
\item \texttt{fir.cpp}: Implements top level function
\item \texttt{fir.h}: Header file
\item \texttt{fir\_test.cpp}: Test bench
\item \texttt{input.dat}: Input chirp signal
\item \texttt{out.gold.dat}: ``Golden'' output. When the testbench (from fir\_test.cpp) is run through the file fir.cpp it should generate this result. If it does not, you did something wrong.
\end{itemize}
\item \texttt{Demo} folder: Demo folder for 11 tap filter
\begin{itemize}
\item \texttt{host\_fir.c}: Unfinished host program
\item \texttt{exe\_script.sh}: Execution script
\item \texttt{plot\_script.p}: Plotting script
\item \texttt{input.dat}: Input chirp signal
\end{itemize}
\item Tutorial folder
\begin{itemize}
\item \texttt{ug871-vivado-high-level-synthesis-tutorial.pdf}: Various tutorials for Vivado HLS
\end{itemize}
\end{itemize}

\section{Project Goal}
The first goal of this project is to generate a design from HLS (FIR11) and implement it on the Zedboard.  Also you should start to gain an understanding of different HLS optimizations. For FIR128, you should modify the code to generate at least four additional architectures. Your goal is to create architectures that provide tradeoffs between area and execution time. This will require you to rewrite the code and/or insert pragmas. Your final assignment must contain followings:
\begin{itemize}
\item Design a 11 tap fir filter with HLS. In the rest of this document, we use the term \term{FIR11} to refer this task.
\item Demo for FIR11: In the rest of this document, we use the term \term{Demo} to refer this task. 
\item Design 128 tap fir filter with HLS and optimize it. In the rest of this document, we use the term \term{FIR128} to refer this subtask.
\end{itemize} 

\section{FIR11}

The first step for the project is to get a functionally correct design working for an 11 tap FIR filter. For this, you will need to use the \VHLS tool, and finish the function body of \texttt{void fir()} in the file \texttt{fir.cpp} to implement the filter. You can test the correctness of your code by using the provided testbench. This code does not need to be highly optimized; you will work on creating optimized code later. It just needs to work correctly. This is the code that you will use to program the programmable logic portion of the Zynq chip on the Zedboard. The next step requires that you set up the Zedboard to run Linux on the ARM processor on the Zynq chip, and communicate data back and forth between the ARM processor and your FIR11 core running on the programmable logic. Further details on this are explained in next section.  

\section{Demo}

Following are steps to implement your FIR11 HLS design on the Zedboard. You will provide the input data (chirp signal) from the ARM, and get the output from the Zedboard to the ARM. To do that, you must write a \texttt{host\_fir.c} program. We provided a template of \texttt{host\_fir.c}. Find the comment \texttt{//Add your code here:} and insert your code after that. You also need to write the gnuplot script to plot the output on the GUI. To do this demo you need: a Zedboard, Mouse, Keyboard, Monitor, and USB Hub.

The specific things you must do in this section are:
\begin{itemize}
\item Download two files from: 
\begin{itemize}
\item \url{http://xillybus.com/downloads/xillinux-eval-zedboard-1.3a.zip}
\item \url{http://xillybus.com/downloads/xillinux-1.3.img.gz}
\end{itemize}
\item Read Sections 1 - 4 in the Xillybus tutorial (\url{http://xillybus.com/downloads/doc/xillybus_getting_started_zynq.pdf}). We will use ISE (not Vivado) in this lab since Xillybus does not play well with the current versions of Vivado.  In other words, follow the instructions in Section 3.5.1 in the Xillybus tutorial to generate your bit stream.
\item Read Part I - IV in the Xillybus HLS integration tutorial (\url{http://xillybus.com/tutorials/vivado-hls-c-fpga-howto-1}), integrate your 11-tap FIR HLS design with Xillybus, and
implement your FIR HLS design on the Zedboard. Finish the given host program \texttt{host\_fir.c}. Again, the functions you need are described in this tutorial. Compile your host program (using \texttt{gcc}). Run \texttt{exe\_script.sh} to get this input/output signal graph. The expected output is as shown in Figure \ref{fig:zillybus_fir_demo}.
\end{itemize}

\begin{figure}
\centering
%\includesvg{images/matrix_vector_sequential}
\includegraphics[width=5.5in]{images/zillybus_fir_demo}
\caption{The expected output for the \texttt{FIR11} demo.}\label{fig:zillybus_fir_demo}
\end{figure}

You should submit the graph with your final write up as proof that you got it to work. We also reserve the right to see the demo in person.

\section{FIR128 Optimization Hints}
You must generate at least one architecture that utilizes all of these optimization hints. This architecture does not have to use all of the hints, e.g., you could generate five different architectures where each one performs one of these optimizations. You are free to use any additional optimizations. The only restriction is that your resulting code is correct, i.e., it matches the golden output.
Some possibilities for optimization include:
\begin{itemize}
\item \textbf{Variable Bitwidths:} The bitwidth of the variables provides a tradeoff between precision, area, and performance. It is possible to specify the exact size of each variable to the tools. Make sure that you do not affect the results, i.e., the output still matches the golden output.
\item \textbf{Removing Conditional Statements:} If/else statements and other conditionals limit the possible parallelism and create additional area. If the code can be rewritten to remove them, it typically makes the resulting architecture smaller and faster.
\item \textbf{Pipelining:} This increases the throughput at the cost of adding area (registers). The area and performance can be varied by changing the initiation interval (II).
\item \textbf{Loop Fission:} Dividing the loop into two or more separate loops may allow for each of those loops to be executed in parallel. This will increase the performance and the area.
\item \textbf{Memory Partitioning:} The storage of the arrays in memory plays an important role in area and performance. On one hand, you could put an array entirely in one memory. And this memory can have a different number of ports (e.g., one or two ports for FPGA block RAM). Or you can divide the array into two or more memories to increase the number of ports. Or you could instantiate each of the variables as its own register, which allows simultaneous access to all of the variables at every clock cycle, but has high area costs. 
\end{itemize}

For your designs, you should report performance and area results. Figure \ref{fig:fir_area_results} and Figure \ref{fig:fir_performance_results} provide an example of how to plot the area and performance results. Figure \ref{fig:fir_area_results} plots the number of LUTs, FFs, DSP, and BRAMs used for 8 different designs. Figure \ref{fig:fir_performance_results} shows the performance in terms of number of FIR outputs/second for these 8 designs.  We describe how we calculate the throughput below. Your graphs do not necessarily have to look exactly like these. These are provided as examples. There are many other ways to present the results. However, it is important to make sure to present the results in the most coherent and organized manner as possible.

\begin{figure}
\centering
%\includesvg{images/matrix_vector_sequential}
\includegraphics[width=5in]{images/fir_area_results}
\caption{The resource usage of eight different FIR architectures.}\label{fig:fir_area_results}
\end{figure}

\begin{figure}
\centering
%\includesvg{images/matrix_vector_sequential}
\includegraphics[width=5in]{images/fir_performance_results}
\caption{The throughput in terms of number of FIR outputs/second of eight different FIR architectures.}\label{fig:fir_performance_results}
\end{figure}

We calculated the throughput of the architectures in terms of number of FIR outputs per second. This requires that we calculate the total time that one call to the \texttt{fir()} function. The throughput is reported in Hz using the formula from Equation 2. We use the ``Estimated Clock Period (ns)'' from HLS report instead of the specified clock period. 

The throughput in Hertz can be calculated as:
\begin{equation}
Throughput (Hz) = \frac{1}{Clock\_Period (s) \cdot Num\_Clock \_Cycles}
\end{equation}                           	
The throughput in MHz can be calculated as:
\begin{align*}
Throughput (Mhz) = \frac{1}{Clock\_Period (s) \cdot Num\_Clock\_Cycles} \cdot \frac{1}{10^6} \\
  		                        = \frac{1000}{Clock\_Period (ns) \cdot Num\_Clock\_Cycles}                    
\end{align*}

You should always present your results using units (Hz, KHz, MHz, etc.) that make ``sense''. For example, you should not do 10000 Hz rather 10 KHz, and 200 KHz instead of .2 MHz.


\note{Remove the following two sections?}
\section{Submission Procedure}

You should submit a report that must include your results for the demo and each of the architecture that you generated for FIR128. For the FIR128, this report should plot the results,  e.g., resource utilization in terms of BRAMs, DSP48, FFs, LUTs, etc., and performance in terms of number of throughput (number of FIR operations/second), clock cycles, clock frequency (which is fixed to 10 ns). Your report should describe each of the architectures that you generated. You should discuss the exact optimization and its resulting architecture. Figures describing the architectures are highly encouraged.

You must also submit your code (and only your code, not other files). Your code should have everything in it so that we can synthesize it directly. This means that you should use pragmas in your code, and not use the GUI to insert optimization directives. Or you can insert the optimizations into your TCL script. We must be able to have all of the knowledge available to easily synthesize any and all of your designs.

The folder should be zipped with a similar file structure as below:
\texttt{FIR\_lab\_LASTNAME1\_LASTNAME2.zip}, where \texttt{LASTNAME2} is included if you are submitting a joint report with another person.

Contents:
\begin{itemize}
\item \texttt{report.pdf}
\item \texttt{demo\_picture}: A screenshot or pdf version of your plot graph from the demo.
\item Folder \texttt{baseline}: original unmodified \texttt{fir.cpp}.
\item Folder \texttt{optimized1} first optimization with \texttt{fir.cpp}.
\item Folder \texttt{optimized2}: second optimized design with \texttt{fir.cpp}
\item \dots
\item Folder \texttt{optimizedN}: nth optimized design with \texttt{fir.cpp}.
\end{itemize}
Each folder also must contain \texttt{script.tcl} file that can be used to create the project

\section{Grading Rubric}
The working demo of your code on the Zedboard will account for 60\% of your grade. You can document this in your report with a screenshot as well as some discussion as to any difficulties that you had during this implementation. Of course, we reserve the right to have you demo this for us in person. The remaining 40\% requires that you generate at least one architecture that uses each of the five listed optimizations (Variable Bitwidths, Removing Conditional Statements, Pipelining, Loop Fission, Memory Partitioning). 

The report should be well written and presented. Additional points (up to 20) will be subtracted for poor reports. Examples of issues include any spelling errors, multiple/egregious grammar, poor presentation of results, lack of written comparison of the results, etc. I expect there to be insights into the different architectures. Simply stating the optimizations that you did and presenting the results is not sufficient. You should attempt to answer questions as to why did this optimization produce better results. Why is one architecture better than the other? What sort of architecture is being generated? Etc. This will help you for future assignments so it is worthwhile spending time understanding the tools now.


==> ofdm_project.tex <==
%% !TeX root = main.tex

\chapter{Orthogonal Frequency-Division Multiplexing (OFDM) Project}
\glsresetall
\label{chapter:ofdm}

\section{Introduction}

In this project, you will learn the very basic idea behind an OFDM system, and implement a simple OFDM receiver in programmable logic.  The project is divided into three parts. The first provides an OFDM transmitter and receiver in Simulink. This gives you insight into the ideas behind OFDM. In the second part, you develop a basic OFDM receiver using HLS. The receiver consists of a \gls{fft} module and a QPSK symbol decoder. The final part is to integrate the receiver onto the  Zedboard using Xillybus to transmit data to the OFDM receiver, and receive the decoded data back from your hardware implementation in the programmable logic. You should use Gplot to show the transmitted and received data as you have done in previous projects.

\section{Part I: Simulink}

We provided a Simulink file with an OFDM transmitter, simulated channel, and receiver design. The goal of this part of the project is to gain an initial understanding of how a very simple OFDM system works. Furthermore, you will use the Simulink file to extract data as a testbench for Parts II and III. In this part, we walk you through a series of steps to familiarize you with Simulink and OFDM. This part is optional in the sense you do not have to turn anything. Though you will need to have at least a decent understand of the Simulink in order to complete the assignments from the next two parts of this project. 

Because the HDL-compatible \gls{fft} block inherently bit-reverses, there are two different Simulink models.
\begin{itemize}
\item Version a: No bit reversal in TX, bit reversal in both HDL and behavioral/algorithmic RX, and thus would provide suitable incoming data for a non-bit-reversing Vivado \gls{fft} receiver.
\item Version b: Bit reversal in TX and in both RX  thus be used with a bit-reversing Vivado \gls{fft} receiver.
\end{itemize}

The simple OFDM transmitter encodes 2-bit data symbol (either values of 0 through 3 or random) onto a digital QPSK modulation pattern. 1024 of these symbols go through a 1024-point blockwise I\gls{fft} and are then converted to floating point and sent over a simulated AWGN channel. Two receiver architectures are provided in parallel: HDL-optimized \gls{fft} and block \gls{fft}. You can synthesize the HDL \gls{fft} into Verilog and then run that through Vivado (not HLS) to obtain FPGA resource use estimates.

\begin{figure}
\centering
\includegraphics[width=5.5in]{images/ofdm_1024a}
\caption{Simulink test bench for a simple OFDM transceiver. This is found in the Simulink file \texttt{hdlcoder\_ofdm\_fft\_eml\_1024b.slx}.}
\label{fig:ofdm_1024a}
\end{figure}

Figure \ref{fig:ofdm_1024a} shows the top level of the provided \texttt{hdlcoder\_ofdm\_fft\_eml\_1024b.slx} file. The 2-bit/symbol data source is at upper left, the transmitter (QPSK + I\gls{fft}) is top center, then the AWGN simulated channel and the OFDM A/D converter. We do everything except the channel math in fixed point, since we are trying to build real hardware. The channel, is not synthesizable into Verilog or hardware, is kept in floating point, in deference to the computational limits of Matlab, which needs to add Gaussian-distributed random numbers to what we transmit into the channel.

Run the simulation and note the resulting bit error rate and scope traces. Note that the transmitter input and the receiver output have been manually time-aligned for you. In a real system this function will be handled by the synchronization correlators (matched filters), such as those we studied in an earlier projects (e.g., Chapter \ref{chapter:phase_detector}). The z-2 block delays the \texttt{Behavioral\gls{fft}} output by two frames = 2048 sample times, to compensate for the 1589 delays through the HDL Optimized \gls{fft}, the 458 delays after it, and one delay for serializer in front of it. You can see from the scope that the two have been aligned by the external delays.

\begin{figure}
\centering
\includegraphics[width=5.5in]{images/ofdm_1024a_scope}
\caption{The first two plots shows signal outputs from two different \gls{fft} paths in \texttt{hdlcoder\_ofdm\_fft\_eml\_1024a}. The third scope plots the difference between these two outputs.}
\label{fig:ofdm_1024a_scope}
\end{figure}
 
The third scope channel is feed from subtractor that compares the two parallel receiver constructs (see Figure \ref{fig:ofdm_1024a_scope}). We did something like this in earlier labs, to provide convenient visual verification that two data streams matched. \textbf{Where is the 2\% error coming from?} Hint: try scoping the respective outputs of the Behavioral\gls{fft} and \gls{fft} HDL Optimized blocks -- if the \gls{fft}s match, then what is causing the disparity?
 
Click on \texttt{Analysis} at the top of your screen, then \texttt{Fixed Point Tool}, then make sure \texttt{hdlcoder\_ofdm\_fft\_eml\_1024a} is selected and change \texttt{Data type override:} to \texttt{[Floating Point] Double [precision]}. What happens to the bit error rate? What is likely going on here?

Important note: Since the hardware-optimized \gls{fft} generates results in bit-reversed order, we have set the block \gls{fft} to do the same. Thus, we compare the (bit-reversed) results from the two receivers, instead of comparing one receiver's output against the original data sequence that was transmitted. We need to add a bit reversal block to the design to do a proper TX-RX bit error rate comparison, but for the moment take the block \gls{fft} as your golden standard.
 
Now lump the \texttt{\gls{fft} HDL Optimized}, \texttt{458-clock delay}, and \texttt{OFDM Receiver Symbol Detection} blocks into a single subsystem (a series of left clicks, one per block, with Shift held down will do nicely), right click on it, and start HDL advisor.
 
Run the resulting Verilog code through Vivado and report projected FPGA resource usage. Do not worry yet about putting this into a Xillybus environment.
 
Now open \texttt{hdlcoder\_ofdm\_fft\_eml\_1024b.slx}. This is similar, except that we are now checking true symbol error rate of recovered data versus originally transmitted data. How were we able to do this, given that the two \gls{fft}s both output bit-reversed data? Also, why are the two error/difference traces on the scope so different? One runs as expected between -3 and +3, but the other has huge spikes of about 255.
 
Describe the two data sources, and try each one in turn by clicking on the \texttt{Manual Switch}. Feel free to invent your own data source generator and to swap it in.  

Important points from this lab:
 
\begin{enumerate}
\item Simplified 1024-point OFDM system with data on every channel.
\item AWGN channel simulation available -- will inject Gaussian noise at a user-selected SNR.
\item Quantization -- we chose 12-bit precision for the receivers' input -- was this enough? What is our practical upper limit of bits? 
\item Bit reversal -- the data emerge from the receiver in bit-reverse order, but we can compensate if we tell the transmitter its incoming data are also in bit-reverse order.
\end{enumerate}

\section{Part II: High Level Synthesis}
The major portion of the OFDM receiver is a 1024-point \gls{fft}. The \gls{fft} is a more efficient version of the Discrete Fourier Transform (DFT). The \gls{fft} utilizes symmetry in the DFT coefficients to provide a recursive implementation that reduces the runtime from O(N2) to O(N log N) where N is the number of samples in the input signal. 

Your tasks for this part of the lab are: 
\begin{enumerate}
\item Implement a working \gls{fft} module that passes the testbench in HLS.
\item Optimize the \gls{fft} module (create and explore multiple architectures) 
\item Implement and optimize the QPSK decoder.
\item Integrate the \gls{fft} and decoder into a complete OFDM receiver.
\end{enumerate}

\subsection{Materials}

You are largely responsible for generating the testbenches for this project. This can be done by extracted data from the provided Simulink file. We do however provide you with testbenches for the \gls{fft}. This is the major part of the receiver.

You are given a zip file with three folders \texttt{0\_Initial}, \texttt{1\_Subcomponents}, and \texttt{2\_Skeleton\_Restructured}.  Folder \texttt{0\_Initial} contains the files corresponding to the ``software'' version of the \gls{fft}. Folder \texttt{2\_Skeleton\_Restructured} provides a framework for a more optimized \gls{fft} implementation. And folder \texttt{1\_Subcomponents} has a number of subfolders that allow you to create projects for individual functions that you will develop over the project. This is largely for your convenience for testing and development. All of the code developed here will eventually be placed in to \texttt{0\_Initial} and \texttt{2\_Skeleton\_Restructured}.
The structure of each of these folders is largely the same.
\begin{itemize}
\item \texttt{*.cpp}: The place where you write your synthesizable code.
\item \texttt{*.h} header file with various definitions that may be useful for developing your code.
\item \texttt{*\_test.cpp}: Testbench
\item \texttt{out.gold.dat}: ``Golden'' output. The testbench (\texttt{*\_test.cpp}) generates a sample input and calls the corresponding function in \texttt{*.cpp} with that sample input. This output of the function is compared to the expected output. This will indicate PASS or FAIL. If it fails, then the code in \texttt{*.cpp} is incorrect.
\item \texttt{script.tcl} and \texttt{directive.tcl}: These allow you to easily create a project. To do this, open the \VHLS Command Prompt tool (\texttt{Start} $\rightarrow$ \texttt{Xilinx Design Tools} $\rightarrow$ \texttt{Vivado HLS} $\rightarrow$ \texttt{Vivado HLS Command Prompt}) and go to the directory where source files and script files reside by using \texttt{cd} command. Then type \texttt{vivado\_hls script.tcl}. This will create a HLS project automatically, so you do not have to add source files, set the top function, select the target device, etc. This will create a folder called \texttt{hls} in that directory with the project. It will also synthesize the project.
\item There is a \texttt{README.txt} which contains a link to the project instructions (this file). \note{probably remove this.}
\end{itemize}

\subsection{Goals}
Part II of the project is divided into stages. The first part of the project is to perform the bit reversal of the input data. Then you optimize a ``software'' version of the code which we have given you (minus the bit reversal portion). After that, you will create a more hardware friendly \gls{fft} architecture. We have provided a testbenches for the individual functions in addition to the testbenches for the overall \gls{fft}. Finally, you must design and implement at QPSK decoder, and integrate it with the \gls{fft} to complete the receiver.

While the major goal of this project is create a functional core, you will also perform optimizations on the code. You should modify the code to create a number of different architectures that tradeoff between performance and area. You will create a report describing how you generated these different architectures (code restructuring, pragmas utilized, etc.). For each architecture you should provide its results including the resource utilization (BRAMs, DSP48, LUT, FF), and performance in terms of throughput (number of \gls{fft} operations/second), latency, clock cycles, clock frequency (which is fixed to 10 ns).

\subsection{\gls{fft} Bit Reversal}
The first step in most optimized \gls{fft} implementation is to reorder the input data by performing ``bit reversed'' swapping. This allows for in-place computation of the \gls{fft}, i.e., the resulting ``frequency domain'' data (as well as the intermediate results) can be stored into the same locations as the input ``time domain'' data. In addition, the output frequency domain data will be in the ``correct order'' at the end of the computation.

An example of the bit reversed data for an 8 point \gls{fft} is shown in Table \ref{tab:bit_reverse}.
\begin{table}[htbp]
\caption{The data for an \gls{fft} must be swapped in a ``bit reverse'' manner. The table shows the decimal value, corresponding binary value, and the reversed binary and decimal values for an 8-point \gls{fft}. }
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
Input & Input  & Reversed  & Reversed  \\
Decimal & Binary & Binary & Decimal \\
Address & Address & Address & Address \\
\hline
0 & 000 & 000 & 0 \\
\hline
1	& 001 &	100	& 4 \\
\hline
2	& 010	& 010	& 2 \\
\hline
3	& 011	& 110	& 6 \\ 
\hline
4	& 100	& 001	& 1 \\
\hline
5	& 101	& 101	& 5 \\
\hline
6	& 110	& 011	& 3 \\
\hline
7	& 111	& 111	& 7 \\
\hline
\end{tabular}
\end{center}
\label{tab:bit_reverse}
\end{table}%

In other words, the input data that was initially stored in the array at location 1 is stored in location 4 after the bit reversal is completed. The input data stored in the array at location 4 will be put in array location 1. The input data stored in locations 0, 2, 5 and 7 stay in those locations. Note that this is only true for an 8 point \gls{fft}. Other sizes of \gls{fft} will have different reordering of the data though it is still based on the bit reversed pattern. For example, in a 16 point \gls{fft}, the input data stored in location 1 (binary 0001) will be relocated into location 8 (binary 1000).

You should create an architecture that, efficiently as possible, transforms the input data into a bit reversed order. Note that there are many ``software'' implementations of this that will not effectively map to ``hardware''. While the first goal is to get a working function, you should also consider the performance of the architecture.

We have given you a set of files that allows you to develop and test this bit reversal code in isolation. This includes a simple testbench that exercises this function directly. You should develop and optimized your bit reversed code here. You will later copy this code into the \gls{fft} code.

This code is in subfolder \texttt{1\_bit\_reverse} in the folder \texttt{1\_Subcomponents}. You should develop your code here to insure that it matches the expected result. Note that this testbench is exercising only one input/output result. In other words, even if it passes this, it may not pass all results. Feel free to add additional testbenches to insure your code is correct.

The bit reverse function has the following prototype: \texttt{void bit\_reverse(DTYPE X\_R[SIZE], DTYPE X\_I[SIZE])}

You should perform the swapping ``in place'' on the data in both of the real and imaginary portions of the data. That is the input data in both \texttt{X\_R} and \texttt{X\_I} will be reordered when the function completes.

Your report should describe your code and its performance and area results. Focus on how you modified your code in order to make it more ``hardware friendly''.

Hint: Logical operations map well to hardware. Calculating the indices of the arrays that should be swapped can be done with logical operations. 

\subsection{Optimizing the ``Software'' Version of the \gls{fft}}
The next portion of this lab performs optimization on a typical software implementation of the \gls{fft}. You are given typical three nested loop implementation of the \gls{fft} in the folder \texttt{0\_Initial}. First, you should understand in detail what this code is doing. It is worth spending time on this now as you will have to rewrite the \gls{fft} in a more hardware friendly manner in the next steps. You can reuse some of this code in those steps.

You should optimize this code as much as possible and detail these optimizations and their performance area results in your report. The results of the code will be poor; it will likely have greater than 250 million cycles. The throughput here is likely much worse than running this in software on a microprocessor. This often happens when we put the initial software versions of an application into a high level synthesis tool. And it should not be all that surprising. The code is optimized to run quickly in software, which runs largely in a sequential model of computation. The code must typically be carefully optimized with the final hardware architecture in mind to get good results. This involves exploiting parallelism and pipelining.

You will also notice that the first loop has function calls to sine and cosine. This code will synthesize quickly with these function calls. However, you may wish to replace these function calls (which will synthesize into CORDIC cores), into table lookups. We have provided two tables in the \texttt{.h} file, \texttt{W\_real} and \texttt{W\_imag} which contain the precomputed twiddle factors for our 1024 \gls{fft}, i.e., \texttt{W\_real[i] = cos(2.0*pi*i/SIZE)} and \texttt{W\_imag[i] = sin(2.0*pi*i/SIZE)} where $i = [0,512)$.

Some potential optimizations include:
\begin{itemize}
\item Using the \texttt{W\_real} and \texttt{W\_imag} tables.
\item Pipelining
\item Loop unrolling
\item Memory partitioning
\end{itemize}

In the report, you should discuss the performance and area numbers of the various optimizations that you apply. This must describe the effect of these optimizations on the architecture, and not just state the optimization that you used.

\subsection{Hardware Friendly \gls{fft} Implementation}

A good architecture will selectively expose and take advantage of parallelism, and allow for pipelining. Your final \gls{fft} architecture will restructure the code such that each stage is computed in a separate function or module. There will be one module for bit reversal that you have already developed, and then $\log N$ stages (10 in our case) for the butterfly computations corresponding to the 2-point, 4-point, 8-point, 16-point, \dots \gls{fft} stages.

The skeleton code for this final \gls{fft} implementation can be found in the \texttt{2\_Skeleton\_Restructured} folder. This creates code connects a number of functions in a staged fashion with arrays acting as buffers between the stages. Figure \ref{fig:staged_fft} provides a graphical depiction of this process.

\begin{figure}
\centering
\includegraphics[width=5.5in]{images/staged_fft}
\caption{A staged implementation of a 1024 \gls{fft}. Bit reversal is followed by 10 stages of butterfly computations. This architecture is capable of pipeline both within the stages and across the stages.}
\label{fig:staged_fft}
\end{figure}

The first step in this process is to create code that computes the first and last stages of the \gls{fft}. The hope is that this will allow you to get a better understanding of exactly how memory accesses and the butterfly computations are performed in a general case. You can develop these two functions \texttt{fft\_stage\_first} and \texttt{fft\_stage\_last} in isolation. They both have subfolders in the \texttt{1\_Subcomponents} folder. Once these are working correctly, you can copy and paste the code directly in the same functions in the \texttt{2\_Skeleton\_Restructured} project.

The next task is to create code that can implement ``generic'' function, i.e., one that can compute any stage of the \gls{fft}. This is the function \texttt{fft\_stages} which also has its own project in the \texttt{1\_Subcomponents} folder. Note that this function prototype is similar to \texttt{fft\_stage\_first} and \texttt{fft\_stage\_last} with one major difference: it has a stage argument. This code will used to implement stages 2 through 9 in the \texttt{2\_Skeleton\_Restructured} project.

Hints:
\begin{enumerate}
\item These stages are performing the same calculation as one iteration of the outer for loop in the \texttt{0\_Initial} project.
\item The major difference between the stages is what data elements you are performing the butterfly functions on, i.e., in what order do you pull data from \texttt{X\_R} and \texttt{X\_I}.
\item Test each of the functions in isolation with the provided projects. Make sure that the code compiles and passes the testbench before attempting any optimizations.
\end{enumerate}

Once you have a correctly functioning set of functions, you should copy and paste them in the \texttt{2\_Skeleton\_Restructured} project and make sure that it passes the testbench. Since our testbenches perform one check, which is far from comprehensive, it is possible, though hopefully unlikely, that you have some error that the \texttt{2\_Skeleton\_Restructured} testbench exposes and was not exercised in the individual testbench. If your code passes the \texttt{2\_Skeleton\_Restructured} project you can assume it is correct (though again since it is only one test, it may be wrong; you should perform significantly more testing if you want this to be anywhere close to production quality).

Now on to the final part of the project, optimizing of this restructured code. You should perform the typical tricks here: pipelining, memory partitioning, unrolling, etc. Some of these may not make sense depending on how you wrote your code. This final architecture should be orders of magnitude better than the \texttt{0\_Initial} project. Highly optimized \gls{fft} architectures can easily have less than 10000 cycles.

You should describe in your report the baseline results and the effects of any optimizations that you performed. By this point, you should be starting to understand what optimizations will work and which will not work, and most importantly why. Describe these insights in your report.

\subsection{QPSK Decoder}
The decoder takes the 1024 I/Q outputs from the \gls{fft} and decodes them into the corresponding binary data. Essentially you have to reverse the encoding that was done in the transmitter. The encoder went from 0 and 1 to -1 and 1. Because you have a perfect channel, the output of your \gls{fft} will be -1 and 1. You must make those into 0 and 1. You can look at the Simulink file to determine the exact encoding. It used a Gray code, and the constellation taken directly from the Simulink file is shown below.

\begin{figure}
\centering
\includegraphics[width=5.5in]{images/qpsk_fft}
\caption{A QPSK constellation using a Gray mapping for translating into the I and Q values.}
\label{fig:qpsk_fft}
\end{figure}

The output of your encoder should be the exact data that was given to the OFDM receiver in the Simulink file. You can create your testbench to reflect this.

\subsection{Receiver Integration}
You should connect the \gls{fft} and the QPSK decoder together to form the complete OFDM receiver. The input to the receiver is the data from the channel. The output of the receiver should match the transmitted data.

\subsection{Optimization Hints and Report Guidelines}

\begin{itemize}
\item You should use a clock period of 10 ns. While varying the clock period can drastically change the results, this is not a focus of this project. Though feel free to modify this and observe the changes. 
\item The output of the various architectures that you generate must match the golden output. We have broken down the project into subcomponents to allow you to develop and test them individually. You would be wise to do it in such a manner.
\item You should not change the data types as given to you. You do not need to perform bitwidth optimization of this project.
\item There are some variable defined in the \texttt{.h} files for you convenience. These include \texttt{SIZE = 1024}, \texttt{SIZE2 = 512}, and \texttt{M = 10} (i.e., $\log$ SIZE). Feel free to use these in your code. They are defined in every \texttt{.h} file across all of the different folders.
\item The major goal of this project is to get fully functional versions of all the code. You should focus more of your time on getting everything to work rather than getting some but not all of the components to work and optimizing them.
\item Your report should describe your code at a high level. Since each of you will likely write different code anyone that reads your report should be able to fully understand what each line of your code does. However, this does not mean that you need to explain each line of code in excruciating detail. It is possible to be succinct and thorough at the same time.
\item The software version has a nested for loop structure that does not allow Vivado HLS to provide an exact number of cycles. The \texttt{tripcount} directive can help with this. You should be able to understand the reported results. For example, while Vivado may give you a best, worst and average case numbers, your algorithm for a fixed size \gls{fft} should be a fixed number of cycles. You should report the exact number of cycles for your throughput numbers. You must describe in your report exactly how you derived your throughput results.
\item You must provide a comparison between the best architecture that you derived using the ``software'' version and the best one using the ``hardware friendly'' framework.
\item It is ok to rewrite the code if it helps you with optimizations. For example, you can change the function interfaces.
\item Your code should be written such that the hardware implementation is optimal. For example, there are many ways to do a bit reversal that are efficient in software but not necessarily efficient in hardware.
\item Comment your code.
\end{itemize}

\section{Part III: Zedboard Demo}
You must implement the entire OFDM receiver on the Zedboard in the programmable logic. You should use Xillybus to transmit data to the receiver, the receiver operates on the data, and you will use Xillybus to get the data off of the programmable logic and back onto the ARM core. You must use Gplot to show that transmitted and the received data. 

You are responsible for extracting the transmitted data from the Simulink testbench. You can use ``To Workspace'' data from any signal in the Simulink file. This will then appear as a variable in the Matlab workspace. There are already several ``To Workspace'' blocks in your Simulink file that you can either use directly or modify to extract the necessary data. You only need to show one ``frame'', i.e., the data from the output of one 1024 \gls{fft}.

We provided the general framework for Gplot, Xillybus, etc. in previous labs. You should use that to create this demo. We will not be providing you with anything more than what was given in previous labs. You should provide a plot similar to Figure \ref{fig:ofdm_zedboard} in your report to prove your design is working.  Please plot the entire 1024-point output. Please also plot a zoomed-in version of the output. We would like to see the ``0 1 2 3 0 1 2 3 0 1 2 3 \dots'' sequence clearly.

\begin{figure}
\centering
\includegraphics[width=6in]{images/ofdm_zedboard}
\caption{An example plot showing the input and output values to the simple OFDM receiver.}
\label{fig:ofdm_zedboard}
\end{figure}


==> phase_detector_project.tex <==
\chapter{Phase Detector Project}
\glsresetall
\label{chapter:phase_detector}

\section{Introduction}

In this lab, you will design the phase detection part of a receiver by implementing a complex FIR filter and a COordinate Rotation DIgital Computer (CORDIC) module. You are going to build a complex FIR filter utilizing four ``real'' FIR filters similar to what you developed in Project 1 (see Chapter \ref{chapter:FIR_Project}).  

The complex FIR filter is used to correlate to a known complex signal.  We use Golay codes which have some great properties related to orthogonality and auto-correlation. This is not important to this lab, but is some really amazing math. I hope you look into it.

The CORDIC function is built from scratch and will likely take a large amount of your time for this assignment. A CORDIC is an efficient method for calculating  trigonometric and hyperbolic functions. CORDIC can do a lot of different functions; we will use it to convert Cartesian coordinates $(x,  y)$ to the polar coordinates $(r, theta)$. 

In the end, you will combine all of these modules into something that is the beginning of a digital communication receiver. The goal is to do simple synchronization and discover the phase of the signal. The output of the CORDIC $(r, theta)$ gives you these results. It is not everything that you need to do, but it is a good start. 

The provided Simulink file gives the transmitter, channel, and receiver. You are building an equivalent receiver in HLS in this project. We used this Simulink project to create the various testbenches for the project.

Finally, you will demonstrate a working system of the complete phase detector using Xilinux on the Zedboard. 

\section{Materials}

The provided folder has a number of subfolders and files corresponding to the different parts of the phase detector.  This contains the documents necessary to build the project. In this folder you will see two folders. One is HLS and other is demo. You will start from HLS folder to design your phase detector using \VHLS.
\begin{itemize} 
\item \texttt{HLS/fir} folder: This folder contains \texttt{*.cpp}, \texttt{*.h}, and script files for a complex FIR filter. The complex is matched filter. You are matching the complex I and Q Golay codes. You can to design the complex FIR filter using your \texttt{fir()} function Project 1. In the \texttt{fir.cpp} file, there are four sub functions \texttt{firI1}, \texttt{firI2}, \texttt{firQ1}, and \texttt{firQ2}. These functions are real FIR filters i.e., the same that you designed in Project 1. You can use your favorite code from Project 1 in these four sub functions. In the complex fir filter, four of these functions are used in the \texttt{fir} function. In that function, you need to connect the four FIR filters \texttt{firI1}, \texttt{firI2}, \texttt{firQ1}, and \texttt{firQ2} to an adder and subtractor to create the complex matched filter. This structure is demonstrated in the Simulink file. 

\item \texttt{HLS/cordic} folder:
\begin{itemize}
\item \texttt{cordiccart2pol.cpp}: The place where you write your synthesizable code. Currently, it only contains the function prototype. 
\item \texttt{cordiccart2pol.h}: Header file with various definitions that may be useful for developing your code.
\item \texttt{cordiccart2pol\_test.cpp}: Testbench
\item \texttt{script.tcl} and \texttt{directive.tcl}: Use this to create your project
\end{itemize}

\item \texttt{HLS/phasedetector} folder: After you design the CORDIC and the complex FIR, you will use them to design the phase detector. 
\begin{itemize}
\item \texttt{fir.cpp}:  Real FIR filter that you designed in Project 1. 
\item \texttt{cordiccart2pol.cpp}: \texttt{cordiccart2pol} function you will design in this project.
\item \texttt{phasedetector.cpp}: Top level skeleton for the phase detector. You use \texttt{fir.cpp} and \texttt{cordiccart2pol.cpp} to design the \texttt{phasedetector} function. 
\item \texttt{phasedetector\_test}: Testbench
\item \texttt{phasedetector.h}: Header file
\item \texttt{script.tcl} and \texttt{directive.tcl}: Use this to create your project
\end{itemize}

\item \texttt{Demo} folder: Demo folder for 11 tap filter
\begin{itemize}
\item \texttt{host.c}: Unfinished host program
\item \texttt{exe\_script.sh}: Execution script
\item \texttt{plot\_script.p}: Plotting script
\item \texttt{input\_i.dat}:Input I signal
\item \texttt{input\_q.data}: Input Q signal

\end{itemize}
\end{itemize}

\section{Tasks}

\begin{figure}
\centering
%\includesvg{images/matrix_vector_sequential}
\includegraphics[width=6in]{images/IQ}
\caption{Input I and Q values to your complex FIR filter.} \label{fig:IQ}
\end{figure}

In this project, you will build a phase detector to process the given I and Q signals shown in Figure \ref{fig:IQ}. The final goal is to implement this phase detector on the Zedboard. To achieve this goal, you will need to finish the following 
tasks:
\begin{enumerate}
\item Implement the complex matched filter and verify it with the given testbench. This matched filter consists of four FIR filter modules which are similar to the ones in your Project 1. For the purpose of debugging, if you plot the outputs of this step, you should expect the waveforms as shown in Figure \ref{fig:XY}.
\item Implement the CORDIC HLS code and verify it with the given testbench.
\item Connect the complex matched filter and CORDIC modules to implement the receiver. Verify this overall design with the given testbench. For the purpose of debugging, if you plot the outputs of this step, you should expect the waveforms as shown in the figure below.
\item Implement the receiver design on the Zedboard. This process is similar to the demo in your Project 1. But this time, we will generate the bit file using Vivado instead of ISE. Please read the ``Hints'' section for some tips about this. The expected output is as shown in Figure \ref{fig:phase_detector_demo}.
\end{enumerate}

\begin{figure}
\centering
%\includesvg{images/matrix_vector_sequential}
\includegraphics[width=6in]{images/XY}
\caption{Output values from the complex FIR filter corresponding to the inputs from Figure \ref{fig:IQ}.}
\label{fig:XY}
\end{figure}

\begin{figure}
\centering
%\includesvg{images/matrix_vector_sequential}
\includegraphics[width=6in]{images/phase_detector_demo}
\caption{Example output plot for the phase detector demo.}
\label{fig:phase_detector_demo}
\end{figure}

The thetas at the R peaks are \texttt{0.015529, 0.047509, 0.079485, 0.111526, 0.143491}, etc.. This is the rotated phases that have been detected by your design.

\section{Hints}

\begin{itemize}
\item Start building the subcomponents and get working versions, i.e., start with \texttt{HLS/fir} and \texttt{HLS/cordic}. Verify them independently.
\item Once you design the \texttt{HLS/fir} and \texttt{HLS/cordic}, move the \texttt{HLS/phasedetector}. 
\item Once you have final functions verified, using the same code start to make the Zedboard demo.
\item Due to Xillybus restrictions, you must use Vivado 2014.1 for the demo. You can use 2014.1 for the entire project.
\item When you synthesize your \texttt{xillybus\_wrapper} HLS project, make sure you set the RTL tool to Vivado (see Figure \ref{fig:xillybus_wrapper}).
\item After you synthesize your \texttt{xillybus\_wrapper} HLS project, you will need to export the RTL. Make sure you follow the settings as specified in Figure \ref{fig:xillybus_settings} when exporting the RTL.
\item To create a Vivado project: In \texttt{xillinux-eval-zedboard-1.3a} $\rightarrow$ \texttt{verilog}, you will find \texttt{xillydemo-vivado.tcl}. In Vivado, click \texttt{Tools} $\rightarrow$ \texttt{Run Tcl Script} to run this tcl file of xillydemo. It will create the Vivado project which is the replacement of the ISE project we used in Project 1.
\item Now you need to import the RTL IP core you exported from your \texttt{xillybus\_wrapper} HLS project to the Vivado design suite.  In \texttt{Project Manager}, click \texttt{IP catalog}, then click \texttt{IP Settings}. In \texttt{IP Settings}, click \texttt{Add IP}. You need to locate the \texttt{xilinx\_com\_hls\_xillybus\_wrapper\_1\_0.zip} file generated by your \texttt{xillybus\_wrapper} HLS project. It is in your \texttt{HLS project folder} $\rightarrow$ \texttt{solution1} $\rightarrow$ \texttt{impl} $\rightarrow$ \texttt{IP}.
\item You will see a folder called \texttt{VIVADO HLS IP} in your IP Catalog view. There is your \texttt{xillybus\_wrapper} IP. Double click it to generate a core of this IP. Keep the default setting in every step of this process. Remember the component name of your IP core, which should be \texttt{xillybus\_wrapper\_0} by default. You can change this component name to anything as long as you use the same name in your \texttt{xillydemo.v} Verilog code.
\item Now, modify \texttt{xillydemo.v} code. This is similar to what you did in Project 1. Again, make sure you use the consistent name where you instantiate your \texttt{xillybus\_wrapper} IP core. 
\item Vivado is very picky about unconnected wires. Therefore, make sure you do not have any unconnected components. Hint: if you do not use xillybus debug, do not instantiate \texttt{fifo\_8x2048} in \texttt{xillydemo.v}.
\item If everything is connected correctly, you should be able to generate the bit file from the Vivado project. 
\end{itemize}

\begin{figure}[!ht]
\centering
%\includesvg{images/matrix_vector_sequential}
\includegraphics{images/xillybus_wrapper}
\caption{Make sure to select Vivado as the design tool.}
\label{fig:xillybus_wrapper}
\end{figure}

\begin{figure}[!h]
\centering
%\includesvg{images/matrix_vector_sequential}
\includegraphics{images/xillybus_settings}
\caption{Required settings for exporting RTL into XIllybus.}
\label{fig:xillybus_settings}
\end{figure}

\section{Report}

Your report should mostly focus on the design of your CORDIC core. For this, I want you to use understand how the precision of the CORDIC core affects the performance and area of your designs. The precision is affected by the number of rotations, and also the bitwidths of the data types, both the data types for the input and output arguments, and the data types of the internal variables. 

You should investigate both of these sources of imprecision by generating a number of different designs. One should plot how the number of rotations affects the performance (throughput/latency) and the area (DSP48s, BRAMS, LUTs, FFs). 

The second source of imprecision is how the number of bits for the fixed point variables that you use. Again, you should investigate how changing the fixed point bits for the variables affects the precision, area, and performance. 

In both cases, you should plot some graphs. Talk about the trends. Give insights into why these trends make sense. Talk about trends or data points that do not make sense.

Some ideas to discuss in your report:
\begin{enumerate}
\item What is the total throughput of your Phase Detector? How does that relate to the individual components (FIR, CORDIC, etc.)? How can you make it better?
\item I am looking for deep insight into the design. Why does the accuracy stop improving after so many iterations? What is the minimal amount of bits required for each variable? Does this depend on the input data? If so, can you characterize the input data to help you restrict the number of required bits? Do different variables require different number of bits?
\item The ultimate goal of the CORDIC is not to use only simple operations, i.e., add and shift. You should not be using divide, multiply, etc. in your CORDIC core.
\item How does the ternary operator \texttt{?} synthesize? Is it useful in this project? 
\end{enumerate}



==> projects.tex <==
\input{fir_project}
\input{phase_detector_project}
\input{dft_project}
\input{ofdm_project}

==> wireless.tex <==





==> wirelessBasics.tex <==
\chapter{Basics of Wireless Communication}
\glsresetall
\label{chap:Wireless}

Wireless systems transmit data over the air using electromagnetic waves. These electromagnetic waves are converted to/from an electrical signal using an antenna. To transmit data, The antenna itself converts data encoded as an electrical signal into an electromagnetic wave which carries the information through the air. On the receive side, the antenna does the opposite; it converts the electromagnetic waves into a voltage across the antenna's terminals. 

The transmitted/received electrical signals are naturally real valued where the value represents the current provided to the antenna's terminals when transmitting or a voltage across the terminal when the systems is in receive mode. The signal can be varied over time in order to transmit information. The exact process used to convey this information is called the modulation. More specifically, modulation changes one or more properties of a high frequency signal which is called the \term{carrier signal}. This involves changing the signal's frequency, amplitude and/or phase. The carrier signal is at a much higher frequency than the data rate, e.g., WiFi uses 2.4 GHz.

Before we go any further on exactly how data is modulated, let us first provide some basic terminology. At its most simplistic form, a \term{signal} is something that conveys information. Mathematically, it is a function that maps a domain into a range. In the case of wireless communication, it is a mapping of time into a voltage or current. A \term{continuous signal} is a function defined of a continuous time interval.  A \term{discrete signal} has values defined at only certain points of time. A continuous signal can be converted into a discrete time signal by \term{sampling} where the \term{sampling interval} defines the time between two consecutive samples. The \term{sampling frequency} is the reciprocal of the sampling interval.  For example, a 1 GHz sampling frequency has a sampling interval of 1 ns. Wireless communication typically employs an \term{analog to digital converter (ADC)} to produce a discrete signal from the received continuous signal. This allows for digital processing of the signal in a general purpose microprocessor, digital signal processor, or FPGA, the latter of which is of course the focus of this book. A \term{digital to analog converter (DAC)} does the reverse; it converts a discrete signal into an continuous signal, e.g., to give to provide a current to the antenna to transmit a signal. 

\section{Modulation}
\label{subsec:modulation}

To convey information using a continuous carrier signal $A_c \cos (2 \pi f_c t + \phi)$, we can change the amplitude $A_c$, the phase $\phi$, and/or the frequency $f_c$. The basic techniques for the transmission of digital information include amplitude shift keying, phase shift keying, and frequency shift keying. Each of these techniques changes the specified portion of the signal in order to transmit a set of 'ones' and 'zeros'. The ``key'' is a discrete value encoded into the signal; in essence it is a transform between the digital (ones and zeros) to analog (carrier signal) domains. 

\begin{aside}
The term ``key'' is derived from Morse code key which is a device that turns something on or off. The straight key is probably the most familiar; it generates an electrical signal when the knob is pressed and is off otherwise.
\end{aside}

\term{Amplitude Shift Keying (ASK)} encodes data using the amplitude of the carrier signal. The simplest form of ASK is called \term{on-off keying} which uses the presence or absence of the carrier signal to represent a ``one'' or ``zero'', respectively. More generally speaking, ASK uses a finite number of amplitude to encode digital data, e.g., using four amplitudes would encode two binary bits.  \term{Phase Shift Keying (PSK)} uses the phase of the carrier signal to encode data. For example, the carrier's phase can be modulated between $0^{\circ}$ and $180^{\circ}$ in order to represent ``one'' and ``zero''. Additional phases can be used to encode more data, e.g., $0^{\circ}$, $90^{\circ}$, $180^{\circ}$, $270^{\circ}$ would represent two binary bits. \term{Frequency Shift Keying (FSK)} modulates the frequency in order to encode data. Binary FSK would use two different frequencies to encode ``zero'' and ``one''. Once again, additional frequencies can be used to encode more data.  Figure \ref{fig:keying} shows how four bits of binary data is encoded into the carrier signal using each of these modulation techniques.  \term{Quadrature Amplitude Modulation (QAM)} modulates both the amplitude and the phase. As such it can be viewed as simultaneously employing ASK and PSK to encode data.  

\begin{figure}
\centering
%\includesvg{keying}
\includegraphics[width=.9\textwidth]{images/keying}
\caption{The ASK, PSK and FSK waveforms representing the binary data `1011'.}
\label{fig:keying}
\end{figure}

The job of the wireless receiver is to demodulate the received signal into a digital data. To do this, we must determine the key parameters of the carrier signal. Consider again the carrier signal $A_c \cos (2 \pi f_c t + \phi)$. Depending on the type of modulation, we need to extract the amplitude $A_c$, the frequency $f_c$, and/or the phase $\phi$. The frequency is the rate of change of the phase, i.e., $f_c$ is the first derivative of $\phi$ with respect to time ($f_c = \frac{\partial \phi}{\partial t}$). Therefore, if we know the amplitude $A_c$ and the phase $\phi$ at every instance of time, we can fully recreate the carrier signal. Because of this sinusoids are often represented using a polar coordinate system as in Figure \ref{fig:polar}. The amplitude of the sinusoid ($A_c$) is the length of the vector while the phase $\phi$ is the angle. The conversion between the polar and Cartesian coordinate system can be done using the trigonometric functions $x = A_c \cos \phi$ and $y = A_c \sin \phi$. The x axis is called the in-phase (I) or real axis portion of the signal while the y axis is called the quadrature (Q) or imaginary portion. 

\begin{figure}
\centering
%\includesvg{keying}
\includegraphics[width=.5\textwidth]{images/polar}
\caption{A polar coordinate representation of a sinusoid. The amplitude of the sinusoid is the length of the vector and the phase is the angle. The x axis is often referred to as the real or in-phase (I) value; similarly the y axis is the imaginary or quadrature (Q) value. }
\label{fig:polar}
\end{figure}

Since we modulate data based upon the amplitude, phase, and frequency, using polar coordinates is a natural way to represent and reasonable about wireless signals. Much of the mathematical foundations behind wireless communications utilize a polar representation. However, the discrete signal provided from/to the ADC and DAC is in terms of Cartesian coordinates, i.e., and I and Q or real and imaginary data. This is due to the fact that it is difficult (and therefore expensive) to change the phase of a high frequency carrier signal using an analog circuit. And it is relatively easy to create an analog circuit that varies the amplitude and phase of signal using I and Q data.

To do this, consider the following trigonometric identity:
\begin{equation}
\cos(u + v) = \cos(u) \cos(v) - \sin(u) \sin(v)
\end{equation}

If we transform the carrier signal using this identity we get:
\begin{equation}
A_c \cos (2 \pi f_c t + \phi) = A_c \cos (2 \pi f_c t) \cos(\phi) - A_c \sin (2 \pi f_c t) \sin(\phi)
\label{eq:carrier_identity}
\end{equation}

Noting that the real or in-phase (I) portion of the carrier signal at any instance of time is $A_c \cos \phi$ while the imaginary or quadrature portion is $y = A_c \sin \phi$ (see Figure \ref{fig:polar}), we can rewrite Equation \ref{eq:carrier_identity} as:

\begin{equation}
A_c \cos (2 \pi f_c t + \phi) = I \cos (2 \pi f_c t)  - Q \sin (2 \pi f_c t)
\end{equation}

The implications of this are that we can modulate the phase of the carrier signal by changing the amplitude of a sine and cosine wave of the same frequency. And therefore we can modify the amplitude, phase, and frequency of a carrier signal by changing the amplitude of a two signals of the same frequency separated by $-90^{\circ}$ phase offset. Or equivalently we can modulate the amplitude, phase, and frequency of a carrier signal using I and Q signals. It is much easier to create a circuit that performs this type of modulation as shown in Figure \ref{fig:IQcircuit}. The circuit requires two mixers (multipliers), a subtractor, and a phase change by $90^{\circ}$. Each of these components are relatively straightforward to design. As such, wireless data is very often represented as in-phase (I) and quadrature (Q).

\begin{figure}
\centering
\includegraphics[width=.5\textwidth]{images/IQcircuit}
\caption{Circuit for generating an RF signal using I and Q data.}
\label{fig:IQcircuit}
\end{figure}

A basic understanding of I\textbackslash{}Q data and the complex plane allows for a better representation of the different modulation techniques. For example, we can denote binary PSK on the complex plane as shown in Figure \ref{fig:bpsk}. A carrier signal with a phase of $0^{\circ}$ encodes a value of `1' while a phase of $180^{\circ}$ denotes a value of `0'.  This is called a constellation diagram. This can be extended to more complex modulation techniques. For example, we can modulate data using both the amplitude and phase. This is called quadrature amplitude modulation (QAM), an example of which is shown in Figure \ref{fig:qam}. Here four bits are encoded into unique amplitudes and phases using a Gray code. The amplitude and phases are arranged into a rectangular fashion, which is common because they are easier to demodulate than other QAM constellations (e.g., circular). Note that BPSK can be considered as a special case of QAM, as can other ASK, PSK and FSK modulations. QAM is a popular modulation technique for higher data rate applications. For example, it is used in digital TV. 


\begin{figure}
\centering
\includegraphics[width=.4\textwidth]{images/bpsk}
\caption{Binary Phase Shift Keying (BPSK) represented on the I\textbackslash{}Q plane using a constellation diagram.}
\label{fig:bpsk}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=.4\textwidth]{images/qam}
\caption{The constellation diagram of a 16 QAM modulation. Four bits are encoded using different phases and magnitudes across the  I\textbackslash{}Q plane.}
\label{fig:qam}
\end{figure}

\note{key relationship between matrices and complex numbers here:  This may help to define terminology from rotations in a 2D plane to complex numbers. Also this could be a series of asides relating these for readers that understand one side or the other. I think that keeping this as rotations and not bringing in complex numbers in this chapter is probably the right idea. } 


\note{I think remove the discussion of complex values and just focus on rotations in an x and y plane.}

\note{It might be useful to have an aside that shows the relationships between I, Q and phase and magnitude. Some formulas calculating with I/Q Signals translating between polar and rectangular form etc.
%Peak Amplitude A = (I?+Q?)?
%Phase Angle ? = tan??(Q/I)
%I = A?cos(?)
%Q = A?sin(?)
%Converting IQ Data to a plain signal: I is the original signal.
%Euler form: A?ei? = A?(cos(?) + i?sin(?)) = I + Qi
}

\note{Need to integrate this. It was moved from CORDIC which was rewritten.}

\note{Key idea: We very often want to view a signal in terms of frequency components. A frequency has an amplitude and phase. We often modulate data onto a signal using three components: amplitude, frequency and phase. Can talk about these three and give examples?}

\note{How does the ``complex'' come into this whole thing? Well through a magical formula called Euler's equation that relates sine and cosines to a complex exponential.}

\note{it is possible to encode information on a sine and cosine separately because they are orthogonal signals.}

\note{Negative frequencies: a ``crazy'' consequence of math? But actually show how there is more information when you consider the complex plane. A cosine can have both a positive and negative frequency. But this cannot be determined until you look at the orthogonal sine value (i.e., the ``imaginary'' portion). The negative frequency is a rotation in the ``opposite'' direction. 
}

Before we dive into the details, recall some basics of complex numbers. When multiplying two complex numbers, their phases add and their amplitudes (magnitudes) multiply. Consider two complex numbers
\begin{equation}
\begin{split} C_1 = I_1 + j \cdot Q_1 = A_1 (\cos \phi_1 + j \cdot \sin \phi_1)  \\
 C_2 = I_2 + j \cdot Q_2 = A_2 (\cos \phi_2 + j \cdot \sin \phi_2)
 \end{split}
\end{equation}
The first part of both equations is the complex number represented in Cartesian coordinates, where the real and imaginary parts are denoted as in-phase (I) and quadrature (Q) values. The second part is in polar form.  

Multiplying these two complex number yields
\begin{equation}
C_1 \cdot C_2 = (I_1 I_2 - Q_1 Q_2) + j \cdot (I_1  Q_2 + I_2  Q_1) = A_1 A_2 (\cos (\phi_1 + \phi_2) + j \cdot \sin(\phi_1 + \phi_2))
\label{eq:add_angle}
\end{equation}
You can see from the polar representation that the multiplication of these two complex numbers results in a summation of their phases (angles) and a multiplication of their amplitudes. Therefore, if we wish to rotate the complex number $C_1$ by some angle, we should multiply it by a second complex number $C_2$ that has a phase of that desired rotation angle. Going forward, we denote the rotating complex number as $C_R$. If we wish to subtract an angle, we can use the complex conjugate of $C_R$, i.e., ${C_R}^{*} = I_R - j \cdot Q_R$. Therefore to subtract the angle of complex number $C_R$ from $C_1$ we perform the complex multiplication
\begin{equation}
C_1 \cdot {C_R}^{*} = (I_1 I_R + Q_1 Q_R) + j \cdot (I_R  Q_1 - I_1  Q_R) = A_1 A_R (\cos (\phi_1 - \phi_R) + j \cdot \sin(\phi_1 - \phi_R))
\label{eq:sub_angle}
\end{equation}
Note the similarities between Equations \ref{eq:add_angle} and \ref{eq:sub_angle}. The major difference is that the signs are flipped in real and imaginary summations of the Cartesian multiply. This shows that the polar multiply performs addition and subtraction of the angles, respectively, as expected. An optimized CORDIC hardware design can take advantage of these similarities. 

\begin{aside}
Complex numbers are a useful representation for digital signal processing because they provide a simple way to model the phase and amplitude of a sinusoidal signal. For more information about this, please see Chapter \ref{subsec:modulation}. Most often in digital communications you will deal with complex numbers since it is easy to generate an analog to digital convertor that provides in-phase (real) and quadrature (complex) data. 

 An \term{imaginary number} was originally derived such that the roots of any polynomial equation, which are defined the solutions to any polynomial equation  
\begin{equation}
x^n + a_1 x^{n-1} + \cdots + a_{n-1} x + a_n
\label{eq:polynomial}
\end{equation}
such that the polynomial equation is equal to zero, i.e.,
\begin{equation}
x^n + a_1 x^{n-1} + \cdots + a_{n-1} x + a_n = 0.
\label{eq:poly_zero}
\end{equation}

Consider the polynomial $x^2 -1$, which we can factor as
\begin{equation}
x^2 - 1 = (x-1)(x+1).
\end{equation} This means the roots are $+1$ and $-1$. In general, if we can factor the polynomial in Equation \ref{eq:polynomial} as
\begin{equation}
x^n + a_1 x^{n-1} + \cdots + a_{n-1} x + a_n = (x - r_1)(x - r_2) \cdots (x - r_n),
\label{eq:poly_factor}
\end{equation} any value such that $x = r_i$ for any $i \in \{1, \cdots, n\}$ satisfies Equation \ref{eq:poly_zero}.

Now consider the polynomial $x^2 + 1$. This has no solution if we only consider real numbers. However, imaginary numbers provide a solution where the root is $\sqrt{-1} = j$. And with the introduction of imaginary numbers we can insure that every polynomial of degree $n$ can be factored into $n$ polynomials of degree one as demonstrated in Equation \ref{eq:poly_factor}.
\end{aside}

Once again, the CORDIC algorithm calculates various trigonometric functions through a set of rotations. First, consider rotating a complex number by $90^{\circ}$. To do this we multiply by $C_R = 0 + j$ since the phase of $C_R = 90^{\circ}$.  By substituting this into Equation \ref{eq:add_angle} and doing some simplification we get
\begin{equation}
C_1 \cdot C_R = - Q_1 + j \cdot I_1 = A_1 (\cos (\phi_1 + 90^{\circ}) + j \cdot \sin(\phi_1 + 90^{\circ}))
\label{eq:plus90}
\end{equation}
which is equivalent to negating the quadrature (imaginary) value of $C_1$ and swapping the in-phase (real) and quadrature values. Note that $A_R = 1$ and thus the amplitude complex number does not change with the rotation.  A similar effect occurs when we want to rotate $C_1$ by $-90^{\circ}$. In this case, we multiply by the complex number $C_R = 0 - j$ which gives us
\begin{equation}
C_1 \cdot C_R = Q_1 - j \cdot I_1  = A_1 (\cos (\phi_1 -  90^{\circ}) + j \cdot \sin(\phi_1 -  90^{\circ}))
\label{eq:minus90}
\end{equation}
which is equivalent to negating the in-phase value of $C_1$ and then swapping the in-phase and quadrature values. Thus, the computation for the rotation by $\pm 90^{\circ}$ is simply a negation and swapping of values which is simple and efficient in an FPGA.

Of course, we also need to efficiently rotate by values other than $90^{\circ}$. To do this, we perform rotations by multiplying by a complex number in the form of 
\begin{equation}
C_R = 1 + j \cdot 2^{-L}
\label{eq:complex_power2}
\end{equation} where $L = 0, 1, 2, 3, ... $ and thus the quadrature value $Q_R = 1, 0.5, 0.25, 0.125, ...$ . This probably seems like an odd choice but it will allow us to efficiently perform the complex multiplication. By substituting Equation \ref{eq:complex_power2} into Equation \ref{eq:add_angle} we get
\begin{equation}
C_1 \cdot C_R = (I_1 - Q_1 \cdot 2^{-L}) + j \cdot (I_1 \cdot 2^{-L} + Q_1) = (I_1 - Q_1 >> L) + j \cdot (I_1 >> L + Q_1)
\end{equation}

Note that calculating both the in-phase and quadrature values is done by a shift and add operation.  Additionally, if $L$ is a constant, then the shift can be implemented with wires in the FPGA, which has almost no resource cost. The rotation of the negative angle, which is done using the conjugate of $C_R$ provides a similarly efficient calculation with shifts and adds
\begin{equation}
C_1 \cdot C_R^{*} = (I_1 + Q_1 \cdot 2^{-L}) + j \cdot (Q_1 - I_1 \cdot 2^{-L}) = (I_1 + Q_1 >> L) + j \cdot (Q_1 - I_1 >> L)
\end{equation}

The next obvious question is what angle are we rotating by? And what about the amplitude of the resulting complex number after the rotation is performed? The phase of a complex number is calculated as 
\begin{equation}
\arctan (\frac{Q}{I})
\end{equation}
and the amplitude as
\begin{equation}
\sqrt{I^2 + Q^2}
\end{equation}
Thus the phase and amplitude of $C_R$ varies as shown in Table \ref{table:complexcordic}. The CORDIC gain is the running change in amplitude of the a complex number ($C_1$) who has gone through the sequential series of rotations of $C_R$ from $L = 0$ to the current value. Thus, the CORDIC gain when $L=0$ is simply the amplitude of $C_R$ when $L=0$, i.e., $| 1 + j | = 1.41421$. The CORDIC gain when $L = 1$ assumes that we have rotated by both $1 + j$, i.e., $C_R$ when $L=0$ and $1 + j \cdot 0.5$, i.e., $C_R$ when $L=1$. Thus the CORDIC gain is the amplitudes of these two $C_R$ numbers multiplied together, $1.41421 * 1.11803 = 1.58114$. You can see that as $L$ increases, the quadrature portion of $C_R$ starts to approach $0$. And as the angle gets smaller, the amplitude approaches $1$, and the CORDIC gain stabilizes to approximately 1.647. 

\note{make sure to look for references to table \ref{table:cordic} and change to \ref{table:complexcordic}.}

\begin{table}[htbp]
\caption{The phase, amplitude, and CORDIC gain of the rotating complex number $C_2$ as L varies.}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
L & $2^{-L}$ 	& $C_R$ 				& $C_R$ Phase ($^{\circ}$) 	& $| C_R |$ 		& CORDIC Gain 	\\ \hline \hline
0 & 1.0 		& $1 + j$  				& 45.000					& 1.41421			& 1.41421		\\ \hline
1 & 0.5 		& $1 + j \cdot 0.5$  		& 26.565					& 1.11803			& 1.58114		\\ \hline
2 & 0.25 		& $1 + j \cdot 0.25$  	& 14.036					& 1.03078			& 1.62980		\\ \hline
3 & 0.125 		& $1 + j \cdot 0.125$  	& 7.125					& 1.00778			& 1.64248		\\ \hline
4 & 0.0625 	& $1 + j \cdot 0.0625$  	& 3.576					& 1.00195			& 1.64569		\\ \hline
5 & 0.03125 	& $1 + j \cdot 0.03125$  	& 1.790					& 1.00049			& 1.64649		\\ \hline
6 & 0.015625 	& $1 + j \cdot 0.015625$  	& 0.895					& 1.00012			& 1.64669		\\ \hline
\end{tabular}
\end{center}
\label{table:complexcordic}
\end{table}%
